Some aspects of impact of the Electron Ion Collider on particle physics at the Energy Frontier

This overview describes several science cases at the Electron-Ion-Collider (EIC) experiment which are traditional to general particle physics. It has an emphasis on connections between future measurements at the EIC and the physics topics explored at high-energy frontier colliders. It covers several selected topics, such as parton density functions, multi-quarks states, correlations of final-state particles, precision QCD measurements and forward jet physics. We will discuss possible EIC measurements that can improve previous experimental results obtained at high-energy (HEP) experiments.

==> sec_bsm.tex <==
\section{Beyond the Standard Model physics}
% (Radja Boughezal, Frank Petriello, Daniel Wiegand)

% text from Sergei
The ability to perform measurements with both polarized electron and proton beams at the EIC provides a powerful tool that can greatly improve probes obtained from the LHC alone.  As an example, we compare the potential constraints on operators in the Standard Model Effective Field Theory (SMEFT) from an EIC with those obtained from Drell-Yan data at the LHC.  We show that EIC data plays an important complementary role since it probes combinations of Wilson coefficients not accessible through available Drell-Yan measurements \cite{Boughezal:2020uwq}. 

Figure~\ref{fig:case1combined} compares the constraints
for the Wilson coefficients from the LHC experiments and the EIC using 10 fb$^-1$ of luminosity. The LHC is not sensitive to certain directions in SMEFT parameter space, while the EIC experiment, due its polarization, can constrains a significant space  of $C_{lq}^{(1)}$ versus $C_{eu}$ values. Thus the EIC experiment is a powerful probe for SMEFT and BSM theories that can impact future searches at the LHC and post-LHC experiments. 


\begin{figure}[h!]
  \centering
    \includegraphics[width=0.9\textwidth]{figs/Case1Combined.pdf}
    \caption{68\% confidence level ellipse in the $C_{lq}^{(1)}$ versus
      $C_{eu}$ space for Case 1 with only LHC data, only EIC data, and
      after combining both experiments. Reproduced from Ref.\cite{Boughezal:2020uwq}}
  \label{fig:case1combined}
\end{figure}


